A Closer Look at Language Model Introspection: Probing Information and Reporting

One way to study language-model introspection is to test whether models can identify where their activations have been perturbed. We train a simple linear classifier to identify the perturbed sentence from the model's activations, then compare its predictions with the model's own answers across pretraining and injection strengths. This tests whether the model is being asked to report information that is already easy to recover. If so, successful localization may be less demanding than it first appears and may not extend to the broader uses that motivate introspection research, such as faithfully explaining a model's reasoning or helping researchers assess the reliability of its answers. With an injection four times the typical activation norm at layer 0 and probe readout at layer 24 in OLMo 3 32B, the supervised probe reaches 98.3 % accuracy after 8.4 billion training tokens, while the model's zero-shot answer remains at chance (11.1 %). At the released base checkpoint, these accuracies reach 99.1 % and 89.6 %, respectively. Across 7B and 32B, location is already decodable in randomly initialized networks, showing that the architecture can support these traces without pretraining. In these experiments, location information lies close enough to the surface for a simple linear probe to recover it, so successful reporting need not imply broader access to the model's internal computation.

==> figures/tab_labels_steps.tex <==
% Clean prompts: share (%) answered with each label, per checkpoint. Label-preference runs.
% \sh shades a cell by its value and leaves zero cells empty.
\definecolor{correctedcolor}{HTML}{2A78D6}
\newcommand{\sh}[1]{\ifnum#1=0 \else\cellcolor{correctedcolor!\the\numexpr#1*6/10\relax}#1\fi}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l*{9}{c}}
\toprule
7B step & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
1k & \sh{6} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{94} \\
5k & \sh{4} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{96} \\
10k & \sh{8} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{70} & \sh{22} \\
20k & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
50k & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
100k & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
200k & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{8} & \sh{90} \\
400k & \sh{0} & \sh{30} & \sh{68} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{2} \\
700k & \sh{2} & \sh{0} & \sh{32} & \sh{1} & \sh{63} & \sh{0} & \sh{0} & \sh{0} & \sh{1} \\
1000k & \sh{0} & \sh{0} & \sh{68} & \sh{32} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
stage 1 end & \sh{14} & \sh{8} & \sh{8} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{2} & \sh{67} \\
stage 2 end & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
base & \sh{84} & \sh{6} & \sh{0} & \sh{1} & \sh{1} & \sh{0} & \sh{0} & \sh{5} & \sh{0} \\
\bottomrule
\end{tabular}\hfill
\begin{tabular}{l*{9}{c}}
\toprule
32B step & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
1k & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
5k & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
10k & \sh{0} & \sh{100} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
20k & \sh{62} & \sh{0} & \sh{38} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} & \sh{0} \\
50k & \sh{22} & \sh{0} & \sh{54} & \sh{19} & \sh{2} & \sh{2} & \sh{0} & \sh{0} & \sh{2} \\
100k & \sh{0} & \sh{0} & \sh{38} & \sh{8} & \sh{10} & \sh{0} & \sh{0} & \sh{0} & \sh{43} \\
200k & \sh{4} & \sh{0} & \sh{4} & \sh{4} & \sh{2} & \sh{3} & \sh{2} & \sh{0} & \sh{81} \\
300k & \sh{4} & \sh{3} & \sh{22} & \sh{7} & \sh{18} & \sh{2} & \sh{16} & \sh{8} & \sh{19} \\
400k & \sh{8} & \sh{20} & \sh{21} & \sh{24} & \sh{14} & \sh{3} & \sh{1} & \sh{8} & \sh{2} \\
500k & \sh{0} & \sh{1} & \sh{62} & \sh{8} & \sh{13} & \sh{6} & \sh{2} & \sh{2} & \sh{5} \\
stage 1 end & \sh{0} & \sh{0} & \sh{16} & \sh{6} & \sh{44} & \sh{5} & \sh{2} & \sh{4} & \sh{24} \\
stage 2 end & \sh{6} & \sh{10} & \sh{26} & \sh{16} & \sh{8} & \sh{2} & \sh{2} & \sh{6} & \sh{23} \\
base & \sh{2} & \sh{0} & \sh{32} & \sh{9} & \sh{16} & \sh{3} & \sh{7} & \sh{4} & \sh{27} \\
\bottomrule
\end{tabular}


==> sections/Expirmentsnotes.tex <==
% Core point
% The information needed to locate an injected sentence is built during pretraining and already sits at the answer position before any post-training. Post-training does not add that information, it adds the answer.
% Experiments



% Probe vs answer across stages (primary). In the base model we train a classifier on the answer position and it finds the injected sentence 83% of the time, the model's own answer is 16%. SFT raises the model's answer to 38% and the classifier does not move through SFT, DPO or Instruct. This is also done going through pretraining, the classifier goes from chance at step 0 to 62-71 in the final base model and the model's answer stays at chance the whole way.

% Retry the primary experiment with a randomly initialized network. The injected sentence is still detectable at the sentence itself (95%), measure at the injection, but nothing reaches the answer position (chance). This shows the carrying is learned by pretraining and not a property of the architecture.

% Few shot. Give the model four worked examples with their answers, then ask it the question. It gives 62%. Examples with the answer format but no injections give 39%.

% No prompt. Give just the nine sentences and check the final token for the information with the probe. 35-40%. Adding the question doubles it. SFT changes nothing.

% Strength. Injection strength is set as a multiple of the average activation norm at the injection layer. Results hold from 2x up and Hahami's injection is 2.0 in these units, so we replicate at their strength.

==> tables/layers_base.tex <==
6 & 22 & 1 & 0 \\
8 & 58 & 2 & 0 \\
12 & 79 & 4 & 0 \\
16 & 72 & 5 & 0 \\
24 & 75 & 5 & 2 \\
32 & 65 & 5 & 2 \\


==> tables/layers_instruct.tex <==
6 & 22 & 1 & 0 \\
8 & 51 & 3 & 0 \\
12 & 72 & 5 & 0 \\
16 & 76 & 4 & 0 \\
24 & 76 & 6 & 2 \\
32 & 71 & 6 & 3 \\


==> tables/layers_sft.tex <==
6 & 20 & 1 & 0 \\
8 & 55 & 3 & 0 \\
12 & 74 & 5 & 0 \\
16 & 79 & 4 & 0 \\
24 & 78 & 5 & 2 \\
32 & 67 & 5 & 3 \\


==> tables/loo.tex <==
vector injected & 95.0 (92.0--99.5) \\
words reversed & 99.8 (99.5--100.0) \\
French sentence & 99.8 (99.5--100.0) \\
off-topic sentence & 100.0 (100.0--100.0) \\
line of code & 99.8 (99.5--100.0) \\
garbled characters & 99.0 (98.5--99.5) \\
repeated sentence & 70.7 (68.0--72.5) \\


==> tables/noprompt.tex <==
Random & 0 & 11.5 & 10.9 \\
Random & 1 & 12.2 & 11.5 \\
Random & 2 & 16.9 & 13.5 \\
Random & 4 & 27.4 & 19.1 \\
Random & 8 & 31.5 & 21.5 \\
Pretrained & 0 & 14.3 & 14.1 \\
Pretrained & 1 & 24.3 & 13.5 \\
Pretrained & 2 & 50.7 & 14.1 \\
Pretrained & 4 & 53.0 & 14.8 \\
Pretrained & 8 & 48.1 & 14.3 \\


==> tables/pretrain.tex <==
1k & 25.0 & 9.2 \\
10k & 45.8 & 11.7 \\
50k & 62.9 & 9.2 \\
150k & 67.1 & 9.2 \\
300k & 66.2 & 8.3 \\
600k & 48.8 & 11.2 \\
final & 82.9 & 17.1 \\


==> tables/stages.tex <==
base & 15.7 (13.9--17.5) & 82.9 (81.9--83.3) \\
sft & 37.5 (35.8--39.4) & 86.2 (85.6--86.9) \\
dpo & 40.8 (37.2--45.6) & 84.7 (83.9--86.1) \\
instruct & 39.4 (36.1--43.9) & 83.9 (82.8--85.6) \\


==> tables/strength_base.tex <==
0.5 & 12 & 14 & 67 & 5 \\
1 & 12 & 15 & 91 & 22 \\
2 & 22 & 51 & 100 & 63 \\
3 & 15 & 63 & 100 & 86 \\
4 & 14 & 65 & 100 & 75 \\
6 & 12 & 51 & 100 & 63 \\
8 & 12 & 37 & 100 & 61 \\


==> tables/strength_instruct.tex <==
0.5 & 15 & 10 & 68 & 7 \\
1 & 20 & 15 & 93 & 25 \\
2 & 70 & 62 & 100 & 76 \\
3 & 76 & 77 & 100 & 88 \\
4 & 67 & 73 & 100 & 76 \\
6 & 55 & 69 & 100 & 55 \\
8 & 53 & 65 & 100 & 57 \\


==> tables/strength_main.tex <==
0.5 & 12 & 14 & 12 & 9 \\
1 & 12 & 15 & 19 & 12 \\
2 & 22 & 51 & 66 & 61 \\
3 & 15 & 63 & 67 & 79 \\
4 & 14 & 65 & 60 & 76 \\
6 & 12 & 51 & 51 & 67 \\
8 & 12 & 37 & 49 & 63 \\


==> tables/strength_sft.tex <==
0.5 & 12 & 9 & 68 & 8 \\
1 & 19 & 12 & 93 & 32 \\
2 & 66 & 61 & 100 & 81 \\
3 & 67 & 79 & 100 & 89 \\
4 & 60 & 76 & 100 & 78 \\
6 & 51 & 67 & 100 & 64 \\
8 & 49 & 63 & 100 & 63 \\

